FlashP: An Analytical Pipeline for Real-time Forecasting of Time-Series Relational Data

Interactive response time is important in analytical pipelines for users to explore a sufficient number of possibilities and make informed business decisions. We consider a forecasting pipeline with large volumes of high-dimensional time series data. Real-time forecasting can be conducted in two steps. First, we specify the part of data to be focused on and the measure to be predicted by slicing, dicing, and aggregating the data. Second, a forecasting model is trained on the aggregated results to predict the trend of the specified measure. While there are a number of forecasting models available, the first step is the performance bottleneck. A natural idea is to utilize sampling to obtain approximate aggregations in real time as the input to train the forecasting model. Our scalable real-time forecasting system FlashP (Flash Prediction) is built based on this idea, with two major challenges to be resolved in this paper: first, we need to figure out how approximate aggregations affect the fitting of forecasting models, and forecasting results; and second, accordingly, what sampling algorithms we should use to obtain these approximate aggregations and how large the samples are. We introduce a new sampling scheme, called GSW sampling, and analyze error bounds for estimating aggregations using GSW samples. We introduce how to construct compact GSW samples with the existence of multiple measures to be analyzed. We conduct experiments to evaluate our solution and compare it with alternatives on real data.

==> paper-exp.tex <==
%!TEX root = paper.tex

\section{Experimental Evaluation}

\subsection{Efficiency}
%
Experiments on speedup via AQP

%%7.1 实验环境
%%30台服务器，每个服务器有96个cpu，512G内存
%%数据集包含两张表 UserProfile, AdTraffic表
%%UserProfile表的schema为(user_id, age, gender, province_id, city_id, occupation, user_level, alipay_amt_avg, alipay_freq, buyer_star_id)
%%ChannelEffect表的schema为(date, channel_id, user_id, impression, click, favorite, cart)
%%实验时通过离线计算将两张表先进行join
%%join后的表名为ChannelUserEffect，schema为(date, channel_id, user_id, impression, click, favorite, cart, age, gender, province_id, city_id, occupation, user_level, alipay_amt_avg, alipay_freq, buyer_star_id)
%%训练集的计算和ARIMA的预测基于ChannelUserEffect表，全量实验数据集包含1亿的用户id，平均每天包含1.5亿条数据

%%7.2 性能测试
%%我们取了5个规模的人群，分别为0.1%, 0.5%, 1%, 5%, 10%，共取了20个query，测试这20个query在binomial sampling不同抽样比例样本下的计算时长。
%%计算时长包含2部分，一部分是计算30天每天的SUM(impression)，另一部分是通过30天的impression次数是用ARIMA模型预测未来30天的impression
%%图1展示了对固定的数据集，在固定的抽样比例下，不同人群规模(selectivity)的计算性能，其中x轴为人群规模，y轴为计算耗时. 
\cfig1: fix the dataset and the sampling rate; (randomly) pick a few queries; x-axis is the selectivity (\ie, number of users satisfying the predicates in the queries); y-axis is the (average) AQP time + time used by the prediction model (using, for example, stacked histograms)
%-----fig1----------
\begin{figure*}[ht]
\begin{minipage}[t]{0.33\linewidth}
\subfigure[Sampling rate 0.1\%]{
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig1-1000.eps}
}
\end{minipage}
% 
\begin{minipage}[t]{0.33\linewidth}
\subfigure[Sampling rate 1\%]{
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig1-100.eps}
}
\end{minipage}
% 
\begin{minipage}[t]{0.33\linewidth}
\subfigure[Sampling rate 10\%]{
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig1-10.eps}
}
\end{minipage}
\caption{**AQP and ARIMA Performance with different selectivity at fixed sampling rate}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------


\cfig2: try a public dataset and repeat \cfig1?

\cfig3: fix the dataset and the sampling rate; (randomly) pick a few queries; x-axis is the number of constraints in the query; y-axis is the (average) AQP time + time used by the prediction model (using, for example, stacked histograms)



\cfig4: try a public dataset and repeat \cfig3?

\cfig5: fix the dataset; (randomly) pick a few queries; x-axis is the sampling rate (from 0.001 to 0.1); y-axis is the (average) AQP time + time used by the prediction model (using, for example, stacked histograms)


%%图2展示了对固定的数据集，在固定的人群规模下(selectivity)，不同抽样比例的计算性能，其中x轴为人群规模，y轴为计算耗时. 
%-----fig2----------
\begin{figure*}[t]
\begin{minipage}[t]{0.33\linewidth}
\subfigure[Selectivity 0.5\%]{
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig5-500000.eps}
% \label{fig:side:a}
}
\end{minipage}
% 
\begin{minipage}[t]{0.33\linewidth}
\subfigure[Selectivity 1\%]{
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig5-1000000.eps}
}
\end{minipage}
% 
\begin{minipage}[t]{0.33\linewidth}
\subfigure[Selectivity 5\%]{
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig5-5000000.eps}
}
\end{minipage}
\caption{AQP and ARIMA Performance with different sampling rate at fixed selectivity (how many rows and days in total? ms?)}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------


\cfig6: try a public dataset and repeat \cfig5?




\subsection{Prediction Precision}
%
How AQP impacts prediction precision

For each experiment, try different datasets (for different ads), and for each dataset, pick a few queries
%%7.3 准确性测试
%%我们研究了不同抽样方法在不同sampling rate以及不同training time stamps上，AQP的误差对ARIMA模型predict result的影响。
%%对于固定的数据集，在固定的sampling rate下，对于不同的抽样方法，我们对每种抽样方法都会抽取100个样本
%%然后使用这100个样本对多个selectivity人群规模的query进行estimate训练数据以及在estimate训练数据上进行arima的预测
%%然后将计算的100个arima预测的forcast，upper_bound,  lower_bound求平均值以及方差


%%图3展示了binomial sampling on impression对于固定的数据集，在固定的人群规模下(selectivity)，进行不同抽样比例进行抽样后的arima预测的误差
%%其中训练周期为180天，预测时长为30天，x轴为抽样比例，y轴为arima预测结果与实际数据的相对误差。
\cfig7: fix the dataset; x-axis is the sampling rate; y-axis is the predication error (group by days in the prediction)

%-----fig3----------
\begin{figure*}[ht]
\subfigure[Selectivity 0.5\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig7-50w_3366106_2_180.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Selectivity 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig7-100w_202210022_2_180.eps}
\end{minipage}
}
\subfigure[Selectivity 5\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig7-500w_718978045_2_180.eps}
\end{minipage}
}
\caption{**ARIMA predict error on impression at different sampling rate}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------






\cfig8: fix the dataset; x-axis is the number of training time stamps; y-axis is the predication error (group by days in the prediction)

%%图4展示了binomial sampling on impression对于固定的数据集，在固定的人群规模下(selectivity)，不同训练周期对的arima预测的误差
%%其中抽样比例为1%，预测时长为30天，x轴为不同训练周期，y轴为arima预测结果与实际数据的相对误差。

%-----fig4----------
\begin{figure*}[hb]
\subfigure[Selectivity 0.5\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig9-500w_718978045_2_100.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Selectivity 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig9-100w_202210022_2_100.eps}
\end{minipage}
}
\subfigure[Selectivity 5\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig9-500w_718978045_2_100.eps}
\end{minipage}
}
\caption{ARIMA predict error on impression at different training time stamps (add sampling rate 0.1\%)}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------




%%图5，6，7，8分别展示了binomial sampling，compressed-arithmetic-mean sampling, compressed-geometric-mean sampling以及uniform sampling
%%对于固定的数据集，在固定的人群规模下(selectivity)，进行不同抽样比例进行抽样后分别在impression, click, favorite以及cart的arima预测的误差以及预测interval
%%其中arima的 训练周期为30天，预测时长为7天，不同抽样方法之间保证的是在固定指标上的数据集样本大小一致。
%%图5,6,7,8(a) x轴为抽样比例，y轴为arima预测结果与实际数据的相对误差。图5,6,7,8(b)x轴为抽样比例，y轴为arima预测的interval。

\cfig9: fix the dataset; x-axis is the selectivity of queries; y-axis is the predication error (group by days in the prediction)

%-----fig5. pv predict relative error and interval----------
\begin{figure*}[ht]
\subfigure[Average prediction error]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig40-50w_129370505_3-30-pv.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Average prediction interval]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig41-50w_129370505_3-30-pv.eps}
\end{minipage}
}
\caption{ARIMA predict error and interval at selectivity 0.5\% (how many queries?) on impression via different sampling methods (add sampling rate 0.005\%? how about AQP error?)}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------


%-----fig6. clk predict relative error and interval----------
\begin{figure*}[ht]
\subfigure[Average prediction error]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig40-50w_129370505_3-30-clk.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Average prediction interval]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig41-50w_129370505_3-30-clk.eps}
\end{minipage}
}
\caption{ARIMA predict error and interval at selectivity 0.5\% on click via different sampling methods}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------


%-----fig7. favorite predict relative error and interval----------
\begin{figure*}[ht]
\subfigure[Average prediction error]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig40-50w_129370505_3-30-col.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Average prediction interval]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig41-50w_129370505_3-30-col.eps}
\end{minipage}
}
\caption{ARIMA predict error and interval at selectivity 0.5\% on favorite via different sampling methods}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------



%-----fig8. cart predict relative error and interval----------
\begin{figure*}[ht]
\subfigure[Average prediction error]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig40-50w_129370505_3-30-cart.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Average prediction interval]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=3.3in, height=3in]{fig/vldb-fig41-50w_129370505_3-30-cart.eps}
\end{minipage}
}
\caption{ARIMA predict error and interval at selectivity 0.5\% on cart via different sampling methods}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------






%%图9,10,11,12分别展示了binomial sampling，compressed-arithmetic-mean sampling, compressed-geometric-mean sampling以及uniform sampling
%%对于固定的数据集，在固定的人群规模下(selectivity)以及固定的抽样比例下分别在impression, click, favorite以及cart指标的预测详情
%其中arima的 训练周期为30天，预测时长为7天，不同抽样方法之间保证的是在固定指标上的数据集样本大小一致。
%%图5,6,7,8(a) x轴为时间，y轴为指标的数据值。


%-----fig9. pv predict case----------
\begin{figure*}[hb]
\subfigure[Sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-5000-pv.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-1000-pv.eps}
\end{minipage}
}
\subfigure[Sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-100-pv.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval at selectivity 5\% (why not 0.5\%? -- inconsistent with 0.5\% above) on impression via different sampling methods (so the predictions in different sampling methods are almost the same?)}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------


%-----fig10. clk predict case----------
\begin{figure*}[hb]
\subfigure[Sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-5000-clk.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-1000-clk.eps}
\end{minipage}
}
\subfigure[Sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-100-clk.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval at selectivity 5\% on click via different sampling methods }
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------



%-----fig11. favorite predict case----------
\begin{figure*}[hb]
\subfigure[Sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-5000-col.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-1000-col.eps}
\end{minipage}
}
\subfigure[Sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-100-col.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval at selectivity 5\%  on favorite via different sampling methods }
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------



%-----fig12. favorite predict case----------
\begin{figure*}[hb]
\subfigure[Sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-5000-cart.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-1000-cart.eps}
\end{minipage}
}
\subfigure[Sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig42-9248224-100-cart.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval at selectivity 5\%  on cart via different sampling methods }
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------




%%图13展示了对于固定的数据集，binomial sampling和compressed-arithmetic-mean sampling保证在没有任何筛选条件下
%%对每一天的impression, click, favorite以及cart四个指标求sum，一共有30天，每一组sample可以获得30个[sum_imp, sum_clk, sum_fav,sum_cart]，每一天共100组
%%对每一天的100组样本求平均，可以每天100组的平均误差，共有30天，再对30天求平均误差，将得到的平均误差来代表样本总体平均AQP误差。
%%实验使得binomial sampling和compressed-arithmetic-mean sampling四个指标参照上面方法，使得总体平均AQP误差接近
%%图13给出了样本的sampling rate和AQP总体平均误差，图14,15分别展示了在上述的样本中，取一个固定selectivity的人群
%%看这个人群在各个指标上的ARIMA predict error and interval
%%16,17,18,19是给出了具体case

%-----fig13. binomial sampling aqp error bound nearly to compressed-arithmetic-mean ----------
\begin{figure*}[hb]
\subfigure[Sampling rate (what is x-axis? AQP error?)]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig1-sample.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[AQP error bound (only one compressed sample, right?)]{
\begin{minipage}[t]{0.5\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig2-3-aqp.eps}
\end{minipage}
}
\caption{Sampling rate via different sampling methods with nearly aqp error bound (can we add uniform and geometric-mean here?)}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------

%%


%-----fig14. predict relative error when binomial sampling aqp error bound close to compressed-arithmetic-mean sampling----------
\begin{figure*}[ht]
\subfigure[Sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2in]{fig/vldb-fig43-500w_9248224_3-100-acc.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2in]{fig/vldb-fig43-500w_9248224_3-1000-acc.eps}
\end{minipage}
}
\subfigure[Sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2in]{fig/vldb-fig43-500w_9248224_3-5000-acc.eps}
\end{minipage}
}
\caption{ARIMA predict error at selectivity 5\%  via different sampling methods with nearly aqp error bound (can we add uniform and geometric-mean here? almost no change for different sampling rates? how can we guarantee that aqp error bounds are nearly the same given the same sampling rate?)}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------


%-----fig15. predict interval when binomial sampling aqp error bound close to compressed-arithmetic-mean sampling----------
\begin{figure*}[ht]
\subfigure[Sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2in]{fig/vldb-fig43-500w_9248224_3-100-gap.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[Sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2in]{fig/vldb-fig43-500w_9248224_3-1000-gap.eps}
\end{minipage}
}
\subfigure[Sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2in]{fig/vldb-fig43-500w_9248224_3-5000-gap.eps}
\end{minipage}
}
\caption{ARIMA predict interval at selectivity 5\% via different sampling methods with nearly aqp error bound (can we add uniform and geometric-mean here? almost no change for different sampling rates? how can we guarantee that aqp error bounds are nearly the same given the same sampling rate?)}
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------



%-----fig16. pv predict case----------
\begin{figure*}[hb]
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-5000-pv.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-1000-pv.eps}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-100-pv.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval on impression at selectivity 5\%  via different sampling methods with nearly AQP error bound }
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------


%-----fig17. clk predict case----------
\begin{figure*}[hb]
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-5000-clk.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-1000-clk.eps}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-100-clk.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval at selectivity 5\%  on click via different sampling methods with nearly AQP error bound }
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------



%-----fig18. favorite predict case----------
\begin{figure*}[hb]
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-5000-col.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-1000-col.eps}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-100-col.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval at selectivity 5\%  on favorite via different sampling methods with nearly AQP error bound }
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------



%-----fig19. favorite predict case----------
\begin{figure*}[hb]
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.02\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-5000-cart.eps}
% \label{fig:side:a}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 0.1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-1000-cart.eps}
\end{minipage}
}
\subfigure[AQP average error nearly Compressed-arithmetic-mean sampling with sampling rate 1\%]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in, height=2.0in]{fig/vldb-fig43-9248224-100-cart.eps}
\end{minipage}
}
\caption{ARIMA average predict error and interval at selectivity 5\%  on cart via different sampling methods with nearly AQP error bound }
% \label{AQP and ARIMA Performance}
\end{figure*}
%---------end-------------





==> paper-proof.tex <==
%!TEX root = paper.tex

\section{Priority v.s. Threshold}
%
Suppose we have $n$ rows with positive measures $m_1, \ldots, m_n$. Each row generates a random variable $\alpha_i \in (0,1)$. The priority \cite{tit:DuffieldLT05,pods:AlonDLT05,jacm:DuffieldLT07} of each row is calculated as $p_i = m_i/\alpha_i$. For a threshold $\tau > 0$, define a random variable $x_i$ for each row:
%
\begin{equation}\label{equ:threshold:variable}
x_i =
	\begin{cases}
	0 & \quad \text{if } \frac{m_i}{\alpha_i} < \tau \\
	\tau & \quad \text{if } m_i < \tau \leq \frac{m_i}{\alpha_i} \\
	m_i & \quad \text{if } \tau \leq m_i \\
	\end{cases}.
\end{equation}
%
In the priority sampling scheme \cite{pods:AlonDLT05,jacm:DuffieldLT07}, $\tau$ is picked to be the $k$th highest priority among all the rows (or a subset of rows).

Let's analyze the distribution of $x_i$. There are two cases:
%
\squishlist
\item Case i) $m_i < \tau$:
\begin{equation}\label{equ:threshold:variable:probability:1}
\begin{cases}
\pr{x_i = \tau} = \frac{m_i}{\tau}
\\
\pr{x_i = 0} = 1 - \frac{m_i}{\tau}
\end{cases}.
\end{equation}
%
\item Case ii) $m_i \geq \tau$:
\begin{equation}\label{equ:threshold:variable:probability:2}
\pr{x_i = m_i} = 1 ~\text{ or }~ \pr{x_i = \tau \cdot \frac{m_i}{\tau}} = 1.
\end{equation}
\squishend

% \stitle{Equivalence to measure-biased sampling.} 
% 
We find that \eqref{equ:threshold:variable:probability:1}-\eqref{equ:threshold:variable:probability:2} are also equivalent to the measure-biased sampling \cite{sigmod:DingHCC016}. Intuitively, if $\tau$ is large enough, each row is {\em selected} ($x_i = \tau$) with probability proportional to $m_i$, as in the first line of \eqref{equ:threshold:variable:probability:1}. In particular, we can construct a measure-biased sample $\cal S$ from a priority sample $\{x_i\}$ as follows: if $x_i = \tau$, put one copy of row $i$ into $\cal S$; if $x_i = m_i$, put $\frac{m_i}{\tau}$ copies of row $i$ into $\cal S$.

\stitle{Estimating (subset) sum.} Define the estimator ${\hat M} = \sum_{i=1}^n x_i$. Indeed, it is unbiased
%
\begin{align*}
\ep{{\hat M}} & = \sum_{i:~m_i < \tau} \ep{x_i} + \sum_{i:~m_i \geq \tau} \ep{x_i}
\\
& = \sum_{i:~m_i < \tau} \tau \cdot \frac{m_i}{\tau} + \sum_{i:~m_i \geq \tau} m_i = \sum_{i=1}^n m_i = M.
\end{align*}

The variance of ${\hat M}$ depends on the value of $\tau$. And indeed, the smaller $\tau$ is, the larger the sample size is. We want to derive the relationship between the variance and the (expected) sample size.

For each $x_i$, in case i) $m_i < \tau$, we have $\vr{x_i} = \ep{x_i^2} - \ep{x_i}^2 = \tau^2 \cdot \frac{m_i}{\tau} - m_i^2 = (\tau - m_i)m_i$; and in case ii) $m_i \geq \tau$, we have $\vr{x_i} = 0$. Since $x_i$'s are independent, we have
\[
\vr{\hat{M}} = \sum_{i=1}^n \vr{x_i} = \sum_{i:~m_i<\tau} (\tau - m_i) m_i.
\]

Regarding the sample size, for a fixed $\tau$, let's define ${\cal S}_{\tau+} = \{i \mid m_i \geq \tau\}$ and ${\cal S}_{\tau-} = \{i \mid \alpha_i \tau \leq m_i < \tau \}$. The sample obtained from \eqref{equ:threshold:variable} is essentially ${\cal S}_\tau = {\cal S}_{\tau+} \cup {\cal S}_{\tau-}$. The set ${\cal S}_{\tau+}$ has a fixed size $|{\cal S}_{\tau+}| = \sum_{i:~m_i \geq \tau} 1$. And the expected size of ${\cal S}_{\tau-}$ is $\ep{|{\cal S}_{\tau-}|} = \sum_{i:~m_i < \tau} \frac{m_i}{\tau}$. Thus, the expected sample size is
\[
\ep{|{\cal S}_\tau|} = \sum_{i=1}^n \frac{\min\{m_i, \tau\}}{\tau} \leq \frac{M}{\tau}.
\]

We can also analyze the relative standard deviation of ${\hat M}$ as in \cite{pods:AlonDLT05}. Simply from its definition, we have
%
\begin{align*}
\ep{\left(\frac{{\hat M}-M}{M}\right)^2} & = \frac{\sum_{i:~m_i<\tau} (\tau - m_i)m_i}{M^2} \leq \frac{\sum_{i:~m_i<\tau} \tau m_i}{M^2}
\\
& = \frac{\tau^2 \ep{|{\cal S}_{\tau-}|}}{M^2} \leq \frac{\ep{|{\cal S}_{\tau-}|}}{\ep{|{\cal S}_{\tau}|}^2} \leq \frac{1}{\ep{|{\cal S}_{\tau}|}},
\end{align*}
%
which is consistent with the main result (\cthm1) of \cite{pods:AlonDLT05}.

